Foundations for Restraining Bolts: Reinforcement Learning with LTLf/LDLf restraining specifications

In this work we investigate on the concept of "restraining bolt", envisioned in Science Fiction. Specifically we introduce a novel problem in AI. We have two distinct sets of features extracted from the world, one by the agent and one by the authority imposing restraining specifications (the "restraining bolt"). The two sets are apparently unrelated since of interest to independent parties, however they both account for (aspects of) the same world. We consider the case in which the agent is a reinforcement learning agent on the first set of features, while the restraining bolt is specified logically using linear time logic on finite traces LTLf/LDLf over the second set of features. We show formally, and illustrate with examples, that, under general circumstances, the agent can learn while shaping its goals to suitably conform (as much as possible) to the restraining bolt specifications.

==> 5-reward-shaping-giuseppe.tex <==
\section{Automata-based reward shaping}

Reward shaping is a well-known technique to guide the agent during the learning process and so reduce the time needed to learn. 
The possibility of using reward shaping in the context of RL  for \LTLf /\LDLf rewards has been exploited in \cite{CamachoCSM17b}. 
%%
The idea is to supply additional rewards in a proper manner such that the optimal policy is the same of the original MDP.
Formally, the original reward $R(s, a, s')$ is replaced by $R'(s, a, s') = R(s, a, s') + F(s, a, s')$, where $F(s, a, s')$ is the \textit{shaping reward function}.
In \cite{Ng:1999:PIU:645528.657613} it has been shown that potential-based reward shaping of the form $F(s, a, s') = \gamma\Phi(s') - \Phi(s)$, for some $\Phi: S \to \mathbb{R}$, is a necessary and sufficient condition for policy invariance under this kind of reward transformation, i.e. the optimal and near-optimal MDP solutions are preserved.

It is crucial to observe that one can define two potential-based reward shaping functions and use them simultaneously by summing the  potential functions.

We observe that,  the use of  reward shaping  when using \LTLf /\LDLf rewards $\varphi$ can be automatized. Given a \LTLf /\LDLf  formula $\varphi$ we build the associated \DFA $\A_\varphi$. This operation is made \emph{off-line}, i.e. before the learning process. Then we associate automatically to the states of the \DFA a potential function $\Phi(q)$ whose value decreases proportionally with the minimum distance between the automaton state $q$ and any accepting state. The potential functions gives a positive reward when the agent performs an action leading to a $q'$ that is one step closer to an accepting state, and a negative one in the opposite case. Moreover, with $\gamma < 1$, a penalty is given if $\Phi(q) = \Phi(q')$.

% We define $\Phi$ over the states of the \DFA $\A_\varphi$ associated to the \LTLf /\LDLf goal formula $\varphi$ so to give a positive reward when the agent performs an action leading to a state $q'$ that is one step closer than $q$ to an accepting state, and a negative one in the opposite case. Moreover, we take into account the results shown in \cite{Grzes:2017:RSE:3091125.3091208}, where the value of $\Phi(q)$ in any terminal state is constrained to zero in order to guarantee policy invariance. \textit{Terminal states} are all the states when in our setting a learning episode can end,
%  namely accepting states (i.e. states where $\forall i.q_i\in F_i$), failure states (i.e. states from where any accepting state is unreachable for some $i$) and the state reached after $N$ actions, where $N$ is the terminal time in a finite horizon scenario. 

 Reward shaping can also be used when the \DFAs of the \LTLf /\LDLf formulas are constructed \emph{on-the-fly} \cite{BDP-AAAI18} so as to avoid to compute the entire automaton off-line. To do so we can rely on \textit{dynamic reward shaping} \cite{Devlin:2012:DPR:2343576.2343638}. The idea is to build $\A_{\varphi}$ progressively while learning. During the learning process, at every step, the value of the fluents $\ell \in \L$ is observed and the successor state $q'$ of the current state $q$ of the \DFA on-the-fly is computed. Then, the transition and the new state just observed are added into the ``built" automaton at time $t$, $\A_{\varphi, t}$, yielding $\A_{\varphi, t'}$. The potential function $\Phi$ for $\A_{\varphi, t'}$ is recomputed for the new version of the automaton. In this case, the shaping reward function takes the following form: $$F(q,t, a,q', t') = \gamma\Phi(q', t') - \Phi(q, t)$$ where $\Phi(q, t)$ is the same of the off-line variant (with some additional heuristics) but computed on the automaton $\A_{\varphi, t}$. Optimality and near-optimality guarantees are still preserved as explained in \cite{Devlin:2012:DPR:2343576.2343638}.

% It is not among the purposes of this work to discuss in detail the different ways to design the potential function, for which we refer to \cite{CamachoCSM17b}. Notice that the potential function is not constrained to be \emph{static}, as described above, but can be \emph{dynamic}, i.e. it might change over time during the learning process. To do so one can rely on \emph{dynamic reward shaping} \cite{Devlin:2012:DPR:2343576.2343638}. In this case, the shaping reward function takes the following form: $$F(q,t, a,q', t') = \gamma\Phi(q', t') - \Phi(q, t)$$ where $\Phi(q, t)$ is the new potential function which depends on automaton state $q$ and time $t$. Optimality and near-optimality guarantees are still preserved as explained in \cite{Devlin:2012:DPR:2343576.2343638}.


\begin{theorem}
	Automata-based reward shaping, both in off-line and on-the-fly variants, preserves optimality and near-optimality of the MDP solutions.
\end{theorem}

% \begin{theorem}
% 	Automata-based reward shaping, both in static and dynamic cases, preserves optimality and near-optimality of the MDP solutions.
% \end{theorem}

\begin{proof} For the off-line case, the shaping-reward function $\Phi$ is, by construction, potential based, hence fulfilling the premises of theorems in \cite{Ng:1999:PIU:645528.657613} and \cite{Grzes:2017:RSE:3091125.3091208}.
	Also for the on-the-fly variant, we observe that our construction is compliant with the requirements shown in \cite{Devlin:2012:DPR:2343576.2343638}.
\end{proof}
%We use automata-based reward shaping in the experiments.

%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% save-place: t
%%% End:


==> reward-shaping.tex <==
\section{Automata-based reward shaping}
Reward shaping is a well-known technique to guide the agent during the learning process and so reduce the time needed to learn. The idea is to supply additional rewards in a proper manner such that the optimal policy is the same of the original MDP.
Formally, the original reward $R(s, a, s')$ is replaced by $R'(s, a, s') = R(s, a, s') + F(s, a, s')$, where $F(s, a, s')$ is the \textit{shaping reward function}.
In \cite{Ng:1999:PIU:645528.657613} it has been shown that potential-based reward shaping of the form $F(s, a, s') = \gamma\Phi(s') - \Phi(s)$, for some $\Phi: S \to \mathbb{R}$, is a necessary and sufficient condition for policy invariance under this kind of reward transformation, i.e. the optimal and near-optimal MDP solutions are preserved.

In our experiments, we use the reward shaping in a straightforward way. Given a \LTLf /\LDLf goal $\varphi$, the associated DFA $\A_\varphi$, the potential function $\Phi(\langle s, q \rangle)$ is computed automatically and its value decreases proportionally with the minimum distance between the automaton state $q$ and any accepting state. The idea is to give a positive reward when the agent performs an action leading to a $q'$ that is one step nearer to an accepting state, and a negative one in the opposite case. 

We also worked on an alternative approach, leveraging the DFA on-the-fly construction associated to a \LTLf /\LDLf formula \cite{BDP-AAAI18} and avoiding to compute the entire automaton off-line and relying on results shown in \cite{Devlin:2012:DPR:2343576.2343638} about \textit{dynamic reward shaping}. The idea is to build $\A_{\varphi}$ progressively, from scratch. During the learning process, at every step, the value of the fluents $\Pi$ is observed and the successor state $q'$ of the current state $q$ of the DFA on-the-fly is computed. Then, the transition and the new state just observed are added into the "learned" automaton at time $t$, $\A_{\varphi, t}$, yielding $\A_{\varphi, t'}$. The potential function $\Phi$ for $\A_{\varphi, t'}$ is recomputed for the new version of the automaton. In this case, the shaping reward function assumes the following form:
$$F(q,t, a,q', t') = \gamma\Phi(q', t') - \Phi(q, t)$$
where $\Phi(q, t)$ is the same of the off-line case (with some additional heuristics) but computed on the automaton $\A_{\varphi, t}$. Optimality and near-optimality guarantees are still preserved even in dynamic reward shaping \cite{Devlin:2012:DPR:2343576.2343638}.

We have taken into account the results shown in \cite{Grzes:2017:RSE:3091125.3091208}, where the value of $\Phi$ in any terminal state is constrained to zero in order to guarantee policy invariance. \textit{Terminal states} are all the states when in our setting a learning episode ends, namely goal states, failure states (i.e. states from where any accepting state is unreachable) and the state reached after $N$ actions, where $N$ is the terminal time in a finite horizon scenario.

\begin{theorem}
	Automata-based reward shaping, both in off-line and on-the-fly cases, preserves optimality and near-optimality of the MDP solutions.
\end{theorem}

Our reward shaping is similar to the one shown in \cite{CamachoCSM17b}, but in our experiments we fully-automated the design of $F$ and seamlessly integrated it in the MDP. Moreover, as shown in the on-the-fly case, we propose an alternative approach that avoids to build the entire automaton off-line, which can be useful when we deal with big size formulas.

%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% save-place: t
%%% End:


==> table1-icaps.tex <==

% Table 1 ICAPS submission

\begin{table}
\begin{tabular}{|c|c|c|c|c|} \hline
{\bf Algorithm} & {\bf Reduced} & {\bf Extended} & {\bf p-value} \\ \hline \hline 

\hline
Sarsa
& 
\begin{tabular}{c}
$\mu$  4897.8  \\
$\sigma$ 1849.3
\end{tabular}
& 
\begin{tabular}{c}
$\mu$ 5028.8 \\
$\sigma$ 903.7
\end{tabular}
&  0.440 \\  \hline

\begin{tabular}{c}
Sarsa($\lambda)$ \\
$\lambda = 0.9$
\end{tabular} 
& 
\begin{tabular}{c}
$\mu$ 4126.3  \\
$\sigma$ 1145.6

\end{tabular}
& 
\begin{tabular}{c}
$\mu$ 4450.9 \\
$\sigma$ 1420.5
\end{tabular}
& 0.323 \\  \hline

\begin{tabular}{c}
$n$-step Sarsa  \\
$n = 10$
\end{tabular} 
& 
\begin{tabular}{c}
$\mu$  10151  \\
$\sigma$ 3174.3
\end{tabular}
& 
\begin{tabular}{c}
$\mu$  9853 \\
$\sigma$ 2981.0
\end{tabular}
&  0.354 \\  \hline

\hline\hline

Sarsa
& 
\begin{tabular}{c}
$\mu$  1305.5  \\
$\sigma$ 359.2
\end{tabular}
& 
\begin{tabular}{c}
$\mu$ 4263.2  \\
$\sigma$ 1535.0
\end{tabular}
&  $6.7 \cdot 10^{-5}$ \\  \hline

\begin{tabular}{c}
Sarsa($\lambda)$ \\
$\lambda = 0.9$
\end{tabular} 
& 
\begin{tabular}{c}
$\mu$ 1094.2  \\
$\sigma$ 338.2
\end{tabular}
& 
\begin{tabular}{c}
$\mu$ 1178.3 \\
$\sigma$ 216.2
\end{tabular}
& 0.296 \\  \hline

\begin{tabular}{c}
$n$-step Sarsa  \\
$n = 10$
\end{tabular} 
& 
\begin{tabular}{c}
$\mu$  2442  \\
$\sigma$ 804.1
\end{tabular}
& 
\begin{tabular}{c}
$\mu$  2696 \\
$\sigma$  653.6
\end{tabular}
&  0.226 \\  \hline

\end{tabular}
\caption{\Sapientino~2 (top) and \Sapientino~3 (bottom) game results. Average  ($\mu$) and standard deviation ($\sigma$) of number of iterations to find a goal policy over 10 experiments for each case ($\gamma = 1$, $\epsilon = 0.1$, $\alpha = 0.01$).}
\label{tab:exp1}
\end{table}



% Table 2 ICAPS submission



\begin{table}
\begin{tabular}{|c|c|c|c|c|} \hline
{\bf Algorithm} & {\bf Reduced} & {\bf Extended} & {\bf p-value} \\ \hline

\begin{tabular}{c}
Sarsa($\lambda)$ \\
$\lambda = 0.99$
\end{tabular} 
& 
\begin{tabular}{c}
$\mu$ 4948.1  \\
$\sigma$ 2531.0

\end{tabular}
& 
\begin{tabular}{c}
$\mu$ 6278.8  \\
$\sigma$ 2270.0
\end{tabular}
& 0.159 \\  \hline

\end{tabular}
\caption{\Breakout game results. Average ($\mu$) and standard deviation ($\sigma$) of number of iterations to find a goal policy over 10 experiments for each case ($\gamma = 1$, $\epsilon = 0.1$, $\alpha = 0.01$).}
\label{tab:exp2}
\end{table}











==> table1-ijcai.tex <==
\begin{table}
\begin{tabular}{|c||c|c||c|c|} \hline
{\bf Goal} & {\bf OP} & {\bf OPC} & {\bf DP}  & {\bf DPC} \\ \hline \hline 

\hline
S2
& 
\begin{tabular}{c}
$\mu$  211.9  \\ % final
$\sigma$ 2.8
\end{tabular}
& 
\begin{tabular}{c}
$\mu$ 212.8 \\ % final
$\sigma$ 3.6
\end{tabular}
&  
\begin{tabular}{c}
$\mu$ 161.7 \\
$\sigma$ 0.7
\end{tabular}
& 
\begin{tabular}{c}
$\mu$ 160.4 \\
$\sigma$ 0.4
\end{tabular}
\\  \hline

\hline
S3
& 
\begin{tabular}{c}
$\mu$  185.5  \\ % final
$\sigma$ 0.05
\end{tabular}
& 
\begin{tabular}{c}
$\mu$  185.3 \\ % final
$\sigma$ 0.3
\end{tabular}
&  
\begin{tabular}{c}
$\mu$  146.7 \\
$\sigma$ 0.4
\end{tabular}
& 
\begin{tabular}{c}
$\mu$ 146.2 \\
$\sigma$ 0.3
\end{tabular}
\\  \hline

\end{tabular}
\caption{\Sapientino game results. Average  ($\mu$) and standard deviation ($\sigma$) (over 10 runs) of highest reward obtained after 10 minutes (\OP and \OPC) and after 40 minutes (\DP and \DPC) of learning.}
\label{tab:exp1}
\end{table}


==> table2-ijcai.tex <==
\begin{table}
\begin{tabular}{|c||c|c||c|c|} \hline
{\bf Goal} & {\bf ML} & {\bf MG} & {\bf FL}  & {\bf FG} \\ \hline \hline 

\hline
LR
& 
\begin{tabular}{c}
$\mu$ 1176    \\
$\sigma$ 179 
\end{tabular}
& 
\begin{tabular}{c}
$\mu$  1112 \\
$\sigma$  369
\end{tabular}
&  
\begin{tabular}{c}
$\mu$  12685 \\
$\sigma$ 147 
\end{tabular}
& 
\begin{tabular}{c}
$\mu$ 10912  \\
$\sigma$ 1213 
\end{tabular}
\\  \hline

\end{tabular}
\caption{\Breakout game results. Average  ($\mu$) and standard deviation ($\sigma$) (over 10 runs) of highest reward obtained after 10 minutes (ML and MG) and after 2 minutes (FL and FG) of learning.}
\label{tab:exp2}
\end{table}

